Towards Effective Planning Strategies for Dynamic Opinion Networks

In this study, we investigate the under-explored intervention planning aimed at disseminating accurate information within dynamic opinion networks by leveraging learning strategies. Intervention planning involves identifying key nodes (search) and exerting control (e.g., disseminating accurate or official information through the nodes) to mitigate the influence of misinformation. However, as the network size increases, the problem becomes computationally intractable. To address this, we first introduce a ranking algorithm to identify key nodes for disseminating accurate information, which facilitates the training of neural network classifiers that provide generalized solutions for the search and planning problems. Second, we mitigate the complexity of label generation, which becomes challenging as the network grows, by developing a reinforcement learning-based centralized dynamic planning framework. We analyze these NN-based planners for opinion networks governed by two dynamic propagation models. Each model incorporates both binary and continuous opinion and trust representations. Our experimental results demonstrate that the ranking algorithm-based classifiers provide plans that enhance infection rate control, especially with increased action budgets for small networks. Further, we observe that the reward strategies focusing on key metrics, such as the number of susceptible nodes and infection rates, outperform those prioritizing faster blocking strategies. Additionally, our findings reveal that graph convolutional network-based planners facilitate scalable centralized plans that achieve lower infection rates (higher control) across various network configurations, including Watts-Strogatz topology, varying action budgets, varying initial infected nodes, and varying degrees of infected nodes.

==> sections/environment_description.tex <==
\section{Environment Description}

In addressing the challenge of misinformation spread within social networks, we formulate our problem within a reinforcement learning (RL) framework. The objective is to develop an RL policy that identifies and influences a 'blocker node' in the network at each timestep. This node, once influenced by official information, stop receiving misinformation. Our approach is grounded in the dynamics of opinion formation and the structural properties of social networks.

\subsection{Network Model}

The network is modeled using the Watts-Strogatz small-world graph to simulate the inter-connections of agents in a social network. This model captures the essence of real-world social structures with its characteristic short path lengths and high clustering coefficient. Within this framework, we explore three distinct cases based on the type of opinion values and trust:

\begin{itemize}
    \item \textbf{Case-1:} Binary Opinion Values with Binary Trust.
    \item \textbf{Case-2:} Floating-Point Opinion Values with Binary Trust.
    \item \textbf{Case-3:} Floating-Point Opinion Values with Floating-Point Trust.
\end{itemize}

\subsection{State Representation}

The state of the environment at each timestep is represented by a combination of the current opinion values of all nodes in the network and the trust relationships between them. Specifically, the state includes:

\begin{itemize}
    \item The opinion vector $\mathbf{x}(t)$, where $x_i(t)$ represents the opinion of node $i$ at time $t$.
    \item The trust matrix $\mu_{ik}$, indicating the level of trust node $i$ has in node $k$.
\end{itemize}

For cases with floating-point trust, the trust matrix is a continuous variable, while for binary trust, it is a binary variable.

\subsection{Action Space}

The action at each timestep involves selecting a blocker node to disseminate authentic information. This selection is based on the current state of the network, aiming to maximize the impact of accurate information spread. The action space is discrete, with each action corresponding to the selection of a single node from the network.

\subsection{Reward Function}

The reward function is designed to encourage policies that effectively mitigate the spread of misinformation. It includes components that penalize the increase in misinformation spread, the number of candidate nodes considered for selection, and rewards strategies that minimize the total time to contain misinformation. Specifically, the reward functions used are:

\begin{itemize}
    \item $R_0 = -(\Delta \text{infection rate})$
    \item $R_1 = -(\text{candidate nodes})$
    \item $R_2 = -(\text{candidate nodes}) - (\Delta \text{infection rate})$
    \item $R_3 = 1 - (\frac{\text{\# time steps}}{\text{Total time steps}})$
    \item $R_4 = -(\text{infection rate})$
\end{itemize}

\subsection{Dynamics of Influence}

Upon the selection of a blocker node, an external source sends official information to this targeted node, influencing its opinion. The influence process continues until the opinion of the blocker node crosses a predefined threshold, ensuring it is immune to misinformation.

\subsection{Training Methodology}

Our model employs an Epsilon-Greedy strategy, balancing exploration with exploitation to effectively navigate the action space. The model architecture is based on a ResNet model, which facilitates the learning of complex patterns in the diffusion of information across the network.

This RL framework, with its detailed state representation, action space, and dynamics of influence, forms the core of our approach to mitigating the spread of misinformation in social networks.


==> sections/methods.tex <==
\paragraph{GNN-based Formulation} 

\begin{algorithm}
\caption{Main Function Pseudocode}
\begin{algorithmic}[1]
\Procedure{Main}{}
    \State $ \textbf{input\_size} \gets 3 $ \Comment{[opinion\_value, degree\_of\_node, proximity\_to\_source\_node]}
    \State $ \textbf{hidden\_size} \gets 64 $
    \State $ \textbf{output\_size} \gets 1 $
    \State $ \textbf{learning\_rate} \gets 0.01 $
    \State $ \textbf{num\_nodes} \gets 400 $
    \State $ \textbf{policy} \gets GCN(input\_size, hidden\_size, output\_size)$ 
    \State $\textbf{optimizer} \gets Adam(learning\_rate)$
    \State $\textbf{criterion} \gets binary\_cross\_entropy\_loss$
    \State $\textbf{loss\_list} \gets {[]}$
    \State $\textbf{episode\_max} \gets 100$

    \\


    \For{$episode \gets 1$ to $episode\_max$} 
        \State $\textbf{graph, node\_features, edge\_index} \gets 
        generate\_graph(num\_nodes)$
        \State \Comment{$\textbf{node\_features} \in \mathbf{R}^{num\_nodes \times  input\_size}$}
        \State $\textbf{total\_loss} \gets 0$
        \State $\textbf{iteration} \gets 0$

        \\

        
        \While{$\text{True}$}
            \State $\textbf{uninfected\_nodes} \gets get\_graph\_properties(graph) $
            \If{$\text{uninfected nodes = 0}$}
                \State $\text{Break}$
            \EndIf
            \State $\textbf{target\_output, blocked\_node} \gets minimize\_infection\_rate(graph) $ 
            \State \Comment $\textbf{target\_output} \gets [t_1, t_2, ..., t_{num\_nodes}]$ where $t_i = 1$ if $i = blocked\_node$ ; $0$ otherwise 
            \State $\textbf{policy\_output} \gets policy(node\_features, edge\_index)$
            \State \Comment $\textbf{policy\_output} \in \mathbf{R}^{num\_nodes \times output\_size}$
            \State $\textbf{loss} \gets criterion(target\_output, policy\_output)$
            \State $\text{Update weights through backpropagation}$
            \State $\textbf{total\_loss} = total\_loss + loss$

            \State \textbf{node\_features}[blocked\_node][0] = -1
            \State $\textbf{graph} \gets update\_graph\_environment(graph)$
            
            \State $\textbf{iteration} = iteration + 1$
        \EndWhile
        \\
        \State $\textbf{total\_loss} = total\_loss / iteration$
        \State $\textbf{loss\_list} =  loss\_list + total\_loss$
    \EndFor
    \State $\text{Save model}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Minimize Infection Rate Pseudocode}
\begin{algorithmic}[1]
\Procedure{MinimizeInfectionRate}{$Graph$}
    \State $\textbf{uninfected\_nodes} \gets \text{get\_graph\_properties}(Graph)$
    \State $\textbf{min\_infection\_rate} \gets 1$
    \State $\textbf{min\_rate\_output} \gets \text{None}$
    \State $\textbf{node\_to\_block} \gets \text{None}$
    \\
    \For{$\text{node in uninfected\_nodes}$}
        \State $\textbf{simulation\_graph} \gets \text{Graph}$
        \State $\textbf{simulation\_graph}[node][0] \gets -1$
        \State $\textbf{infection\_rate} \gets \text{SimulatePropagation}(simulation\_graph)$
        \If{$\text{infection\_rate} < \text{min\_infection\_rate}$}
            \State $\textbf{min\_infection\_rate} \gets \text{infection\_rate}$
            \State $\textbf{min\_rate\_output} \gets [0]^{Graph.num\_nodes \times 1}$ 
            \State $\textbf{min\_rate\_output}[node] \gets 1$
            \State $\textbf{node\_to\_block} \gets \text{node}$
        \EndIf
    \EndFor
    \\
    \State \Return $\text{min\_rate\_output}, \text{node\_to\_block}$
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Simulate Propagation Pseudocode}
\begin{algorithmic}[1]
\Procedure{SimulatePropagation}{$Graph$}
    \State $\textbf{number\_of\_nodes}, \textbf{infected\_nodes}, \textbf{blocked\_nodes}, \textbf{uninfected\_nodes} \gets \text{get\_graph\_properties}(Graph)$
    \State $\text{visited\_nodes} \gets \text{[]}$
    \\
    \Procedure{DFS}{$node, parent$}
        \If{$\text{node in visited\_nodes or Graph[node][0] == -1}$}
            \State \Return
        \EndIf
        \State $\text{visited\_nodes.insert(node)}$
        \If{$\text{parent in infected\_nodes and node not in infected\_nodes}$}
            \State $\text{infected\_nodes.append(node)}$
        \EndIf
        \For{$\text{neighbor in Graph.neighbors(node)}$}
            \State $\text{DFS(neighbor, node)}$
        \EndFor
    \EndProcedure
    \\
    \For{$\text{source\_node in infected\_nodes}$}
        \If{$\text{source\_node not in visited\_nodes}$}
            \State $\text{DFS(source\_node, -1)}$
        \EndIf
    \EndFor

    \\
    \State $\textbf{num\_infected\_nodes} \gets \text{len(set(infected\_nodes))}$
    \State $\textbf{proportion\_infected\_nodes} \gets \text{num\_infected\_nodes / number\_of\_nodes}$
    \State \Return $\text{proportion\_infected\_nodes}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Update Graph Environment Pseudocode}
\begin{algorithmic}[1]
\Procedure{UpdateGraphEnvironment}{$Graph$}
    \State $\text{infected\_nodes} \gets \text{[]}$ \Comment{Initialize an empty list to store infected nodes}
    \For{$\text{node in Graph.nodes}$} \Comment{Iterate over all nodes in the graph}
        \If{\text{Graph[node][0]} $ = 1$} \Comment{Check if the node is infected}
            \State $\text{infected\_nodes.insert(node)}$ \Comment{Append the infected node to the list}
        \EndIf
    \EndFor
    \\

    \State \Comment{Calculate updated opinion value}
    \State $\text{updated\_this\_iteration} \gets \text{[]}$
    \For{$\text{node in infected\_nodes}$}
        \For{$\text{neighbor in Graph.neighbors(node)}$}
            \If{$\text{neighbor in updated\_this\_iteration}$}
                \State \textbf{continue}
            \EndIf
            \If{$\text{Graph[neighbor][0] != -1}$}
                \State \textbf{diff} = Graph[node][0] - Graph[neighbor][0]
                \State $\text{Graph[neighbor][0]} \gets \text{min}(1, Graph[neighbor][0] + \text{diff})$
                \State $\text{updated\_this\_iteration.append(neighbor)}$
            \EndIf
        \EndFor
    \EndFor

    \\

    \State \Comment{Calculate updated degree}
    \For{$\text{node in Graph.nodes}$}
        \State $\text{Graph[node][1]} \gets \text{Graph.degree[node]}$
        \For{$\text{neighbor in Graph.neighbors(node)}$}
            \If{$\text{Graph[neighbor][0] in [-1, 1]}$}
                \State $\text{Graph[node][1]} \gets \text{Graph[node][1] - 1}$
            \EndIf
        \EndFor
    \EndFor

    \\
    \State \Comment{Calculate updated shortest paths}
    \For{$\text{node in Graph.nodes}$} 
        \If{$\text{Graph[node][0] == 1}$} 
            \State $\text{Graph[node][2]} \gets 0$ 
            \State \textbf{continue} 
        \ElsIf{$\text{Graph[node][0] == -1}$} 
            \State $\text{Graph[node][2]} \gets \text{Graph.number\_of\_nodes()}$
        \EndIf
        \State $\text{Graph[node][2]} \gets \text{BFS(Graph, node)}$ 
    \EndFor
    
    \State \Return $\text{Graph}$
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Breadth-First Search Pseudocode}
\begin{algorithmic}[1]
\Procedure{BFS}{$Graph, current\_node$}
    \State $\textbf{visited} \gets \text{Set}()$ \Comment{Initialize an empty set to store visited nodes}
    \State $\textbf{queue} \gets \text{Queue}(current\_node)$ \Comment{Initialize a queue with the current node}
    \State $\textbf{distances} \gets \text{Dict}(current\_node, 0)$ \Comment{Initialize a dictionary to store distances}
    \State $\textbf{shortest\_path} \gets \text{Graph.numberOfNodes}()$ \Comment{Initialize the shortest path length}
    
    \\
    
    \While{$\text{queue is not empty}$}
        \State $\textbf{node} \gets \text{queue.pop()}$ 
        
        \\
        
        \If{$\text{Graph[node][0] == 1}$} 
            \If{\text{distances[node]}$ < $ \text{shortest\_path}}
                \State $\text{shortest\_path} \gets \text{distances[node]}$
            \EndIf
            \State \textbf{continue}
        \EndIf

        \\

        
        \For{$\text{neighbor in Graph.neighbors(node)}$}
            \If{$\text{neighbor not in visited and Graph[neighbor][0] != -1}$}
                \State $\text{visited.add(neighbor)}$ 
                \State $\text{queue.insert(neighbor)}$ 
                \State $\text{distances[neighbor]} \gets \text{distances[node] + 1}$
            \EndIf
        \EndFor
    \EndWhile
    \State \Return $\text{shortest\_path}$ 
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Graph Convolutional Network (GCN) Pseudocode}
\begin{algorithmic}[1]
\Procedure{GCN}{$input\_size, hidden\_size, output\_size$}
    \State $\textbf{layer1} \gets \text{GCNConv}(input\_size, hidden\_size)$ 
    \State $\textbf{layer2} \gets \text{GCNConv}(hidden\_size, hidden\_size)$ 
    \State $\textbf{layer3} \gets \text{GCNConv}(hidden\_size, output\_size)$ 
    \State $\textbf{layer4} \gets \text{Linear}(output\_size, output\_size)$ 
    \State $\textbf{sigmoid} \gets \text{Sigmoid()}$ 
\EndProcedure

\\

\Procedure{forward}{$node\_features, edge\_index$}
    \State $\text{output} \gets \text{layer1}(node\_features, edge\_index)$ 
    \State $\text{output} \gets \text{ReLU}(output)$ 
    \State $\text{output} \gets \text{layer2}(output, edge\_index)$ 
    \State $\text{output} \gets \text{ReLU}(output)$ 
    \State $\text{output} \gets \text{layer3}(output, edge\_index)$ 
    \State $\text{output} \gets \text{ReLU}(output)$
    \State $\text{output} \gets \text{layer4}(output)$
    \State $\text{output} \gets \text{sigmoid}(output)$
    \State \Return $\text{output}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\paragraph{Supervised vs Reinforcement Learning}

\paragraph{Classical Planning} 
